Integrated Luminosity with 100 ppm Precision, Methods for $\sqrt{s}$ Precision of 1 ppm, and Beyond Standard Model Sensitivity using Photonic Events, at $\mathrm{e^{+}e^{-}}$ Higgs Factories

Future electron-positron ($\ee$) colliders, operating as Higgs factories or Z factories, promise unprecedented precision electroweak measurements that are vital to testing the Standard Model (SM) and exploring physics beyond it. Here we present work on the precision of integrated luminosity ($\mathcal{L}$) and center-of-mass energy ($\sqrt{s}$), measurements that are needed to make future precision measurements possible. We also conduct these studies for the International Linear Collider (ILC) from the Z pole ($m_{Z}$) to 1~TeV to provide a comprehensive study of these issues for future $\ee$ colliders. Paths to 100 parts-per-million (ppm) precision on $\mathcal{L}$ are presented, with focus on small-angle Bhabha scattering (SABS) and two-photon production (diphotons, $\gamma\gamma$). Previous studies found that beam deflection of SABS events introduce biases on $\mathcal{L}$ of $10^{-2}$. To address this, we present a novel method that uses M\o{}ller scattering with SABS to measure beam deflection and minimize its effect on $\mathcal{L}$. We present a proposal for a Highly Granular Luminosity Calorimeter, the GLIP LumiCal, and its design considerations. We demonstrate that the GLIP LumiCal can achieve $\approx35$ ppm precision on $\mathcal{L}$ precision with diphotons for all values of $\sqrt{s}$ and that the current LumiCal design is insufficient for reaching 1000 ppm. Multiple methods for precision $\sqrt{s}$ estimation are presented. We introduce the use of Kernel Density Estimation (KDE) to ensure that $\sqrt{s}$ is measured accurately and precisely The utility of photon measurements is extended to photon with invisible ($X^0\gamma$) events where we demonstrate methods to measure left-handed and right-handed neutrino couplings and put constraints on Beyond Standard Model (BSM) physics.

==> DefTab.tex <==
\begin{table}
\centering
\caption{Collection of the results of simulating beam deflection for ILC at various center-of-mass energies. This was done with \Gls{SABS} simulated from BHLUMI and within the acceptance of the ILD \Gls{LumiCal}. There was no cut on the acollinearity of the \Gls{SABS} events generated by BHLUMI. The deflection was measured using the net bias across the minimum and maximum acceptance polar angles. Quoted uncertainties are reflective of 1M samples.}
\label{tab-defvals}       % Give a unique label
% For LaTeX tables you can use
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{5}{|c|}{\textbf{Beam Deflection of SABS Events at ILC}}\\
\hline
\textbf{$\sqrt{s}$ (GeV)} & \textbf{$\mathrm{e}^-$ $\theta$ Bias (nrad)} & \textbf{$\mathrm{e}^-$ $\phi$ Bias (nrad)} & \textbf{$\mathrm{e}^+$ $\theta$ Bias (nrad)} & \textbf{$\mathrm{e}^+$ $\phi$ Bias (nrad)} \\\hline
91.2 & 0.6 $\pm$ 1.5  & 20.4 $\pm$ 31.4 & 1.5 $\pm$ 1.5 & 1.0 $\pm$ 41.4 \\
162.4 & -  & - & - & \\
250& -  & - & - & \\
500& -  & - & - & \\
1000& 2.1 $\pm$ 1.5 & 19.8 $\pm$ 31.1 & -1.2 $\pm$ 1.5 & 9.4 $\pm$ 43.2\\\hline
\end{tabular}
% Or use
%\vspace*{1cm}  % with the correct table height
\end{table}
